Demystifying the DAO Governance Process

Decentralized Autonomous Organization (DAO) becomes a popular governance solution for decentralized applications (dApps) to achieve decentralized governance. In the DAO, no single entity can arbitrarily control the dApps without approval from the majority of members. However, despite its advantages, DAO has also been targeted by several attacks, leading to the loss of millions of dollars. In this paper, we first provided an overview of the DAO governance process within the blockchain. Next, we identified the issues within three components of governance process: Governance Contract, Documentation, and Proposal. Each of these components is vulnerable to issues that could potentially result in substantial financial losses. Then we developed automated methods to detected above issues. To investigate the issues within the existing DAO ecosystem, we constructed a state-of-the-art dataset that includes 16,427 DAOs, 183 documentation, and 122,307 proposals across 9 different blockchains. Our analysis reveals that a majority of DAO developers and members have not given sufficient attention to these issues, especially in the area of proposal. The result shows that over 60% of the examined proposals fail to provide a consistent description and code for their members, highlighting a significant gap in ensuring transparency within the DAO governance process. For a better DAO governance ecosystem, DAO developers and members can utilize the methods to identify and address issues within governance process.

==> motivation.tex <==
\section{Motivation}


\subsection{Motivation Example}
In this section, we will exhibit the risk factors within each component of the governance process and corresponding issues by giving the corresponding test cases.

For the governance contract, since it controls the whole DAO governance process. It is required by the defination~\cite{ETH_WP}

The malicious developer can hide some privilege functions in the governance contract that are controlled by themself rather than the governance contract. So that they can adopt these functions to interpreter the governance process, so that the integrity of the proposal result can be violated. From example, the governance contract "0x41E6......7a42" within "mini dao" from DAO type Tally. The function "setVotingPeriod" "setProposalThreshold" and "setVotingDelay" is controlled by a EOA address specified by the developer rather than the governance contract itself. Thus, the developer can arbitrary control the governance process by passing or cancel any proposal by setting the voting delay to 0, priod and threshold to a small value, like one block, so that the developer can vote for a proposal and immediately set voting delay to 0 so that no one can vote for the proposal.


% RQ1
% DAO "0x41E6dC2CC382125c86D9DeDD31359f20785d7a42" from polygon
% % 73bd3e92ffdf6b8c5c16034d19de85b0120d7364
% from Tally 
% Close source
% Only allow external address to setVotingDelay(uint256) setVotingPeriod setProposalThreshold. So that the admin can set the threshold to any value to cancel a proposal or pass a proposal

RQ2 
Compound provide detail documentation for DAO member to participate into the governance process, like Member Participation Voting Power Governance Process Guide.
Guide user to fully interactive proposal, as shown in the Figure~\ref{fig:Compound_doc}

\begin{figure}
\begin{center}
\includegraphics[width=1 \columnwidth]{./image/CompoundDemo.png}
\end{center}
\caption{The Compound documentation for DAO members to vote for proposals.}\label{fig:Compound_doc}
\end{figure}


% DAO has doc proposal numbers, DAO without propsoal numbers

RQ3 for the DAO proposals, the YAM attack that once passed will violates the 3.1 million dollars lost. The proposal
\begin{figure}
\begin{center}
\includegraphics[width=1 \columnwidth]{./image/governance_attack_example.png}
\end{center}
\caption{The malicious within YAM governance attack}\label{fig:YAM}
\end{figure}
"iption :
Contributors comps for May, backpay for VDM, settling synths tokens and success tokens, sending settled rewards tokens to reserves, sending and withdrawing test uma and claiming sushi for reserves."

while "\_setPendingGov(address)"
